Repurposing GANs for One-shot Semantic Part Segmentation

While GANs have shown success in realistic image generation, the idea of using GANs for other tasks unrelated to synthesis is underexplored. Do GANs learn meaningful structural parts of objects during their attempt to reproduce those objects? In this work, we test this hypothesis and propose a simple and effective approach based on GANs for semantic part segmentation that requires as few as one label example along with an unlabeled dataset. Our key idea is to leverage a trained GAN to extract pixel-wise representation from the input image and use it as feature vectors for a segmentation network. Our experiments demonstrate that GANs representation is "readily discriminative" and produces surprisingly good results that are comparable to those from supervised baselines trained with significantly more labels. We believe this novel repurposing of GANs underlies a new class of unsupervised representation learning that is applicable to many other tasks. More results are available at https://repurposegans.github.io/.

==> content/UNUSED_3method2.tex <==
% \section{Method}
% Our problem concerns semantic part segmentation with the following novel setup. Given an image dataset of objects from a single object class and part annotations for only $k$ images, our goal is to segment an unseen object from the same class by learning from very few training labels down to $k=1$. Part annotations in each of the $k$ training images are given as per-pixel masks. For example, for human faces, there could be 3 binary masks, each specifying pixels for the eyes, nose, and mouth. Note that semantic part segmentation can also be considered as an $n$-way \emph{per-pixel} classification problem where $n$ is the number of parts.

% This problem would become trivial if there exists a function $f$ that maps each pixel value, which lacks semantic meaning by itself, to its own feature vector that contains discriminative information for part classification. We propose to derive such a function from a GAN trained to synthesize images of the target class. In the following sections, we will explain how GANs are utilized for this task, how to use the computed per-pixel features for segmentation, and a novel pipeline that allows fast segmentation without reliance on GAN and its expensive mapping.

% %However, GANs can not be used directly as our mapping function simply because . 

% %In this section, we explain our pipeline which has two main procedures: (1) GANs' representation extraction and (2) image segmentation with the extracted representation as input. %The key ideas of our method is that all spatial information from the representation must be preserved.
% %Given the pre-trained network, we produce the semantic segmentation result by this two steps: 
% \subsection{Representation Extraction from GANs}
% Using GANs as a mapping function is not straightforward simply because GANs take as input a random latent code, not the image pixels to be mapped. To understand our process, first consider a typical scenario where we generate an image by feeding a random latent code to a convolutional-based GAN. In this case, the synthesized output image is constructed by the generator through a series of spatial convolutions, and each output pixel is a result of a unique generative computation that can be traced back through each convolution layer down to the initial latent code. Our key idea is to use these \emph{computational paths} for feature representation. 
% %In other words, we are representing each pixel using a sequence of activation values used to produce that pixel.
% In particular, we extract the activation map from every layer (or some subset of layers) from the generator and upsample each activation map to the size of the output using bilinear interpolation. These activation maps are then concatenated in the channel dimension and together represent a feature map of size $H\times W \times C$ where $C$ is the number of activation maps combined from all layers. This process maps each 3-dimensional RGB pixel to a $C-$dimensional feature vector which corresponds to a sequence of spatially-aligned activation values within the generator.

% This extraction of feature map is only possible for images that are synthesized by the generator and thus cannot be used directly for real test images. However, given any test image, one can optimize for a latent code that generates that given test image with any gradient-based optimization or with more sophisticated schemes \todo{cites}. The resulting latent code then allows the feature map to be constructed in a similar manner.




% %To extract the features from GANs and use them as the representation, most existing works use only the single output from the network (e.g., the output from the final convolution layer of classifier network, the bottleneck output of the encoder-decoder based network), or use multiple layers separately. To capture knowledge from all layers as well as their spatial information, we propose the way to extract the representation as follows:\\

% %We call those kinds of representation a global representation. Even though the global representation contains some useful information, it lacks the spatial knowledge which is hypothesized to affect the performance of the semantic segmentation. To retain as much spatial information in the transferred representation, we propose the way to extract the representation as follows: \\

% %Given the pre-trained GANs which consists of a sequence of convolution layers, we extract the output from every blocks of convolution layer and its activation function. Since the output from each block has different spatial dimension, we use bilinear interpolation to upsample every output into the same dimension which equals the dimension of the largest output. Then, we constructed the representation by concatenating all outputs together over the channel dimension.

% \subsection{Segmentation with Extracted Representation}
% To solve segmentation, we first train a GAN on images of the class of interest and generate $k$ random images by feeding it random latent codes. Then, we compute feature maps and manually annotate object parts for these $k$ images. The $k$ feature maps and annotations together form our supervised training pairs which can be used to train a neural network such as a multilayer perceptron or a convolutional network. To segment a test image, we compute a pixel-wise feature map for the test image using the aforementioned latent code optimization and feed it directly to our trained network.

% \subsection{Secondary Segmentation Network}
% Explain UNET.
% %After we get the representation, we input it into the segmentation network, which is the non-linear classifier that predicts per-pixel object classes.\\
% %\indent In this work, we use 2 different structures of segmentation networks throughout the experiments: Multilayer perceptron-based network(MLP) and Convolution-based network (CNN). %We use images and segmentation ground truth from CelebAMask-HQ dataset \cite{CelebAMask-HQ}.
% \todo{Move to implementation details}
% \begin{itemize}
% \item For MLP, we use 2 hidden layers MLP with the number of nodes 2,000 and 200 for the first layer and the second layer respectively.
% \item For CNN, linear embedding was used to downscale the large dimension of representation. We then applied repeated pairs of dilated convolution layer and leaky-ReLU until the channel dimension of the result is equal to the number of object classes. 
% \end{itemize}
% Both MLP and CNN were trained for 1,000 iterations using Adam optimizer with an initial learning rate of 0.001 which was reduced by a factor of 10  every 50 iterations. We also use 0.001 of weight decay to prevent over-fitting. 


% \iffalse
% The method is formulated as: \\
% \indent Given the network $N: \textbf{x} \rightarrow \textbf{y}$ where $\textbf{x}$ and $\textbf{y}$ are input and out of the network respectively.  $N$ consists of sequence of $n$ convolution layers, $f_{i}$ for $i=0,1,2,...,n-1$ so that $\textbf{y}$ can be written as $$\textbf{y} = f_{n-1}f_{n-2}f_{n-3}...f_{0}(\textbf{x})$$ We extract the feature map $r_{i}$ from each convolution, $$r_{i} = f_{i}(\textbf{p})$$ where $\textbf{p} = f_{i-1}f_{i-2}f_{i-3}...f_{0}(\textbf{x})$ and $r_{i} \in \mathbb{R}^{H_{i}\times W_{i}\times C_{i}}.$
% \indent Since each $r_{i}$ has different spatial dimension $H_{i}$ and $W_{i}$, we upsample each $r_{i}$ to $r_{i}^{\prime} \in \mathbb{R}^{\hat{H}\times \hat{W}\times C_{i}}$ where $\hat{H} = \max_{n}H_{i}$ and $\hat{W} = \max_{n}W_{i}$. Then we concatenate each $r_{i}^{\prime}$ channel-wise to produce the pixel-wise representation $$\textbf{r} = r_{0}^{\prime}\oplus r_{1}^{\prime}\oplus r_{2}^{\prime}\oplus... \oplus r_{n-1}^{\prime}$$ 
% where $\textbf{r} \in \mathbb{R}^{\hat{H}\times \hat{W}\times\sum_{n} C_{i}}.$
% Finally, we input those pixel-wise representations into the segmentation model to predict the segmentation map.
% \fi


